A study of first-passage time minimization via Q-learning in heated gridworlds

Optimization of first-passage times is required in applications ranging from nanobots navigation to market trading. In such settings, one often encounters unevenly distributed noise levels across the environment. We extensively study how a learning agent fares in 1- and 2- dimensional heated gridworlds with an uneven temperature distribution. The results show certain bias effects in agents trained via simple tabular Q-learning, SARSA, Expected SARSA and Double Q-learning. While high learning rate prevents exploration of regions with higher temperature, low enough rate increases the presence of agents in such regions. The discovered peculiarities and biases of temporal-difference-based reinforcement learning methods should be taken into account in real-world physical applications and agent design.

==> IEEE Access NoiseRL for Arxiv/algorithms/double_learning.tex <==
\begin{algorithm}
% \KwResult{Write here the result }
\DontPrintSemicolon
\SetAlgoNoLine
 Initialize $Q^A(s, a)$, $Q^B(s, a)$, $S$ \;
 \Repeat{\upshape done}{
  Choose $A$ based on $Q^A(S,\cdot)$ and $Q^B(S, \cdot)$, observe $R$ and $S'$ \;
  Choose random UPDATE(A) or UPDATE(B) \;
  \uIf{\upshape UPDATE(A)}{
     Define $a^\star = \argmax_a Q^A(S, a)$\;
     $Q^A(S, A) \leftarrow Q^A(S, A) + \alpha \ \big( r + \gamma \ Q^B(S', a^\star) - Q^A(S, A)\big)$ \;
   }
   \uElseIf{\upshape UPDATE(B)}{
     Define $b^\star = \argmax_a Q^B(S, a)$\;
     $Q^B(S, A) \leftarrow Q^B(S, A) + \alpha \ \big( r + \gamma \ Q^A(S', b^\star) - Q^B(S, A)\big)$ \;
   }
   $S \leftarrow S'$
 }
 \caption{Double Q-learning \cite{hasselt2010double}}
 \label{algo:double_learning}
\end{algorithm}

==> IEEE Access NoiseRL for Arxiv/algorithms/expected_sarsa.tex <==
\begin{algorithm}
% \KwResult{Write here the result }
\DontPrintSemicolon
\SetAlgoNoLine
 Initialize $Q(s, a)$, $S$ \;
 \Repeat{\upshape done}{
  Choose $A$ from $\varepsilon$-greedy policy \;
  Take action $A$, observe $R$ and $S'$ \;
  $Q(S, A) \leftarrow Q(S, A) + \alpha \ \big( R + \gamma \ \mathbb{E}_{\pi}\big[ Q(S', a)\big] - Q(S, A)\big)$ \;
   $S \leftarrow S'$
 }
 \caption{Expected SARSA \cite{john1994expected_sarsa}}
 \label{algo:expected_sarsa}
\end{algorithm}

==> IEEE Access NoiseRL for Arxiv/algorithms/q_learning.tex <==
\begin{algorithm}
% \KwResult{Write here the result }
\DontPrintSemicolon
\SetAlgoNoLine
 Initialize $Q(s, a)$, $S$ \;
 \Repeat{\upshape done}{
  Choose $A = \argmax_a Q(S, a)$ or with $\varepsilon$ probability choose random $a$ \;
  Take action $A$, observe $R$ and $S'$ \;
  $Q(S, A) \leftarrow Q(S, A) + \alpha \ \big( r + \gamma \ \max_a Q(S', a) - Q(S, A)\big)$ \;
   $S \leftarrow S'$
 }
 \caption{Q-learning with $\varepsilon$-greedy policy \cite{watkins1992q}}
 \label{algo:q-learning}
\end{algorithm}

==> IEEE Access NoiseRL for Arxiv/algorithms/sarsa.tex <==
\begin{algorithm}
% \KwResult{Write here the result }
\DontPrintSemicolon
\SetAlgoNoLine
 Initialize $Q(s, a)$, $S$\;
 Choose $A$ from $\varepsilon$-greedy policy\;
 \Repeat{\upshape done}{
  Take action $A$, observe $R$ and $S'$ \;
  Choose $A'$ from $\varepsilon$-greedy policy \;
  $Q(S, A) \leftarrow Q(S, A) + \alpha \ \big(R + \gamma \ Q(S', A') - Q(S, A)\big)$ \;
   $S \leftarrow S'$, $A \leftarrow A'$
 }
 \caption{SARSA \cite{rummery1994sarsa}}
 \label{algo:sarsa}
\end{algorithm}

==> IEEE Access NoiseRL for Arxiv/tables/table_1D.tex <==
\begin{table}[H]
  \caption{The most common policy $\pi_Q$, $10^4$~agents, $\alpha$~=~0.1, learning~time~=~50k time frames}
  \label{table:1D}
  \centering
  \begin{tabular}{l l l l l} 
    \toprule
      &  & \multicolumn{3}{c}{Right actions,\%} \\
    \cmidrule(r){3-5}
    T & $\pi_Q$ & $x_0$ & $x_0 - 1$ & $x_0 - 2$ \\
    \midrule
    0 & $\pi_0$ & 50 & 0 & 0 \\
    1 & $\pi_R$ & \orange{99} & 0 & 0 \\
    2 & $\pi_R$ & \orange{97} & 0 & 0 \\
    3 & $\pi_{RR}$ & \green{100} & \red{75} & 0 \\
    4 & $\pi_{RR}$ & \green{100} & \red{91} & 0 \\ 
    5 & $\pi_{RR}$ & \green{100} & \red{96} & 1 \\ 
    6 & $\pi_{RR}$ & \green{100} & \red{100} & 1 \\ 
    7 & $\pi_{RR}$ & \green{100} & \red{100} & \red{50} \\ 
    8 & $\pi_{RR}$ & \green{100} & \red{100} & \red{41} \\ 
    9 & $\pi_{RRR}$ & \green{100} & \red{100} & \red{95} \\ 
    10 & $\pi_{RRR}$ & \green{100} & \green{100} & \red{80}\\
    \bottomrule
  \end{tabular}
\end{table}

==> IEEE Access NoiseRL for Arxiv/tables/table_1D_drift.tex <==
\begin{table}[H]
  \caption{Q-learning for the case with drift: $10^4$~agents, $\alpha$~=~0.1, learning~time~=~50k~time steps, difference between policies: MC $10^4$ runs. Right actions are suboptimal.}
  \label{table:drift}
  \centering
%   \begin{tabular}{lllp{0.35\linewidth}}
  \begin{tabular}{llll}
    \toprule
    T & drift & $\displaystyle\frac{\pi_R - \pi_L}{\pi_L}$, \% & $\substack{\text{Right} \\\text{actions in $x_0$}}, \%$ \\
    % T & drift & $\displaystyle\frac{\pi_R - \pi_L}{\pi_L}$, \% & Right actions in $x_0$, \% \\
    \midrule
 1 & 0.10 & 4.3 & 75 \\
   & 0.15 & 6.7 & 31 \\
   & 0.20 & 9.5 & 10 \\ 
    \midrule
 2 & 0.10 & 3.7 & 67 \\
   & 0.15 & 5.9 & 36 \\ 
   & 0.20 & 8.3 & 16 \\
    \midrule
 3 & 0.10 & 0.5 & 99 \\ 
   & 0.15 & 2.2 & 96 \\ 
   & 0.20 & 3.7 & 94 \\ 
   & 0.25 & 5.9 & 86 \\ 
   & 0.30 & 7.5 & 68 \\
   & 0.35 & 9.2 & 42 \\
   & 0.40 & 12.0 & 25 \\
%   & 0.45 & 14.2 & 8 \\ [0.7ex]
    \bottomrule
\end{tabular}

\end{table}

==> IEEE Access NoiseRL for Arxiv/tables/table_1D_drift_ieee.tex <==
\begin{table}[H]
  \caption{Q-learning for the case with drift: $10^4$~agents, $\alpha$~=~0.1, learning~time~=~50k~time steps, difference between policies: MC $10^4$ runs. Right actions are suboptimal.}
  \label{table:drift}
  \setlength{\tabcolsep}{4pt}
  \centering
  \begin{tabular}{|p{10pt} p{25pt} p{50pt} p{80pt}|}
    \hline
    T & drift & $\displaystyle\frac{\pi_R - \pi_L}{\pi_L}$, \% & Right actions in $x_0$, \% \\
    \hline
 1 & 0.10 & 4.3 & 75 \\
   & 0.15 & 6.7 & 31 \\
   & 0.20 & 9.5 & 10 \\ 
    \hline
 2 & 0.10 & 3.7 & 67 \\
   & 0.15 & 5.9 & 36 \\ 
   & 0.20 & 8.3 & 16 \\
    \hline
 3 & 0.10 & 0.5 & 99 \\ 
   & 0.15 & 2.2 & 96 \\ 
   & 0.20 & 3.7 & 94 \\ 
   & 0.25 & 5.9 & 86 \\ 
   & 0.30 & 7.5 & 68 \\
   & 0.35 & 9.2 & 42 \\
   & 0.40 & 12.0 & 25 \\
%   & 0.45 & 14.2 & 8 \\ [0.7ex]
    \hline
\end{tabular}

\end{table}

==> IEEE Access NoiseRL for Arxiv/tables/table_1D_ieee.tex <==
\begin{table}[H]
  \caption{The most common policy $\pi_Q$, $10^4$~agents, $\alpha$~=~0.1, learning~time~=~50k time frames}
  \label{table:1D}
  \centering
  \begin{tabular}{|p{10pt} p{25pt} p{30pt} p{30pt} p{30pt}|} 
    \hline
      &  & \multicolumn{3}{c}{Right actions,\%} \\
    \cmidrule(r){3-5}
    T & $\pi_Q$ & $x_0$ & $x_0 - 1$ & $x_0 - 2$ \\
    \hline
    0 & $\pi_0$ & 50 & 0 & 0 \\
    1 & $\pi_R$ & \orange{99} & 0 & 0 \\
    2 & $\pi_R$ & \orange{97} & 0 & 0 \\
    3 & $\pi_{RR}$ & \green{100} & \red{75} & 0 \\
    4 & $\pi_{RR}$ & \green{100} & \red{91} & 0 \\ 
    5 & $\pi_{RR}$ & \green{100} & \red{96} & 1 \\ 
    6 & $\pi_{RR}$ & \green{100} & \red{100} & 1 \\ 
    7 & $\pi_{RR}$ & \green{100} & \red{100} & \red{50} \\ 
    8 & $\pi_{RR}$ & \green{100} & \red{100} & \red{41} \\ 
    9 & $\pi_{RRR}$ & \green{100} & \red{100} & \red{95} \\ 
    10 & $\pi_{RRR}$ & \green{100} & \green{100} & \red{80}\\
    \hline
  \end{tabular}
\end{table}

==> tables/table_1D.tex <==
\begin{table}[H]
  \caption{The most common policy $\pi_Q$, $10^4$~agents, $\alpha$~=~0.1, learning~time~=~50k time frames}
  \label{table:1D}
  \centering
  \begin{tabular}{l l l l l} 
    \toprule
      &  & \multicolumn{3}{c}{Right actions,\%} \\
    \cmidrule(r){3-5}
    T & $\pi_Q$ & $x_0$ & $x_0 - 1$ & $x_0 - 2$ \\
    \midrule
    0 & $\pi_0$ & 50 & 0 & 0 \\
    1 & $\pi_R$ & \orange{99} & 0 & 0 \\
    2 & $\pi_R$ & \orange{97} & 0 & 0 \\
    3 & $\pi_{RR}$ & \green{100} & \red{75} & 0 \\
    4 & $\pi_{RR}$ & \green{100} & \red{91} & 0 \\ 
    5 & $\pi_{RR}$ & \green{100} & \red{96} & 1 \\ 
    6 & $\pi_{RR}$ & \green{100} & \red{100} & 1 \\ 
    7 & $\pi_{RR}$ & \green{100} & \red{100} & \red{50} \\ 
    8 & $\pi_{RR}$ & \green{100} & \red{100} & \red{41} \\ 
    9 & $\pi_{RRR}$ & \green{100} & \red{100} & \red{95} \\ 
    10 & $\pi_{RRR}$ & \green{100} & \green{100} & \red{80}\\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/table_1D_drift.tex <==
\begin{table}[H]
  \caption{Q-learning for the case with drift: $10^4$~agents, $\alpha$~=~0.1, learning~time~=~50k~time steps, difference between policies: MC $10^4$ runs. Right actions are suboptimal.}
  \label{table:drift}
  \centering
%   \begin{tabular}{lllp{0.35\linewidth}}
  \begin{tabular}{llll}
    \toprule
    T & drift & $\displaystyle\frac{\pi_R - \pi_L}{\pi_L}$, \% & $\substack{\text{Right} \\\text{actions in $x_0$}}, \%$ \\
    % T & drift & $\displaystyle\frac{\pi_R - \pi_L}{\pi_L}$, \% & Right actions in $x_0$, \% \\
    \midrule
 1 & 0.10 & 4.3 & 75 \\
   & 0.15 & 6.7 & 31 \\
   & 0.20 & 9.5 & 10 \\ 
    \midrule
 2 & 0.10 & 3.7 & 67 \\
   & 0.15 & 5.9 & 36 \\ 
   & 0.20 & 8.3 & 16 \\
    \midrule
 3 & 0.10 & 0.5 & 99 \\ 
   & 0.15 & 2.2 & 96 \\ 
   & 0.20 & 3.7 & 94 \\ 
   & 0.25 & 5.9 & 86 \\ 
   & 0.30 & 7.5 & 68 \\
   & 0.35 & 9.2 & 42 \\
   & 0.40 & 12.0 & 25 \\
%   & 0.45 & 14.2 & 8 \\ [0.7ex]
    \bottomrule
\end{tabular}

\end{table}
